The Dynamic Behavior of Frameless ALOHA: Drift Analysis, Throughput, and Age of Information

We study the dynamic behavior of frameless ALOHA, both in terms of throughput and age of information (AoI). In particular, differently from previous studies, our analysis accounts for the fact that the number of terminals contending the channel may vary over time, as a function of the duration of the previous contention period. The stability of the protocol is analyzed via a drift analysis, which allows us to determine the presence of stable and unstable equilibrium points. We also provide an exact characterization of the AoI performance, through which we determine the impact of some key protocol parameters, such as the maximum length of the contention period, on the average AoI. Specifically, we show that configurations of parameters that maximize the throughput may result in a degradation of the AoI performance.

==> Figures/colour_map_AM.tex <==
% define line-styles
\tikzstyle{dashed} 	= [dash pattern=on 8pt off 5pt]
\tikzstyle{dashed_dense} 	= [dash pattern=on 5pt off 1.5pt]
\tikzstyle{dashddotted} 	= [dash pattern=on 11pt off 3pt on \the\pgflinewidth off 3pt on \the\pgflinewidth off 3pt on \the\pgflinewidth off 3pt]
\tikzstyle{dashdotted} 	= [dash pattern=on 7pt off 3pt on \the\pgflinewidth off 3pt]
\tikzstyle{dottedAM}	= [dash pattern=on 2pt off 4pt]



% definition of several colours

%
%\definecolor{col_A}{HTML}{332288}
\definecolor{col_B}{HTML}{88CCEE}
\definecolor{col_C}{HTML}{44AA99}
\definecolor{col_D}{HTML}{117733}
\definecolor{col_E}{HTML}{999933}
\definecolor{col_F}{HTML}{DDCC77}
\definecolor{col_G}{HTML}{CC6677}
\definecolor{col_H}{HTML}{882255}
\definecolor{col_I}{HTML}{AA4499}
\definecolor{col_J}{RGB}{239,151,8}
\definecolor{col_K}{HTML}{56B4E9}
\definecolor{col_A}{RGB}{133,149,225}

\definecolor{darkRed}{RGB}{142,6,59}
\definecolor{mildBlue}{RGB}{133,149,225}
\definecolor{strongerPink}{RGB}{211,63,106}
\definecolor{lightRed}{RGB}{187,119,132}
\definecolor{strongPink}{RGB}{224,123,145}
\definecolor{lightPink}{RGB}{247,156,212}

% gray-scale and tones around it
\definecolor{graphite}{HTML}{594D5B}
\definecolor{grey}{HTML}{6D616F}
\definecolor{silver}{HTML}{ADADC9}
\definecolor{pebble}{HTML}{333333}
\definecolor{coin}{HTML}{9897A9}
\definecolor{dove}{HTML}{7C6E7F}
\definecolor{rust}{HTML}{A4969F}
\definecolor{cloud}{HTML}{C5C6D0}


% new values
\definecolor{AM_col1}{HTML}{ed553d}
\definecolor{AM_col2}{HTML}{b20f58}
\definecolor{AM_col3}{HTML}{ffa600}
\definecolor{AM_col4}{HTML}{5b065c}

\definecolor{AM_s2c1}{HTML}{e0537f}
\definecolor{AM_s2c2}{HTML}{b957a1}
\definecolor{AM_s2c3}{HTML}{2b66ad}
\definecolor{AM_s2c4}{HTML}{3886e3}
\definecolor{AM_s2c5}{HTML}{9673d3}

